Kohn-Sham equations as regularizer: building prior knowledge into machine-learned physics

Including prior knowledge is important for effective machine learning models in physics, and is usually achieved by explicitly adding loss terms or constraints on model architectures. Prior knowledge embedded in the physics computation itself rarely draws attention. We show that solving the Kohn-Sham equations when training neural networks for the exchange-correlation functional provides an implicit regularization that greatly improves generalization. Two separations suffice for learning the entire one-dimensional H$_2$ dissociation curve within chemical accuracy, including the strongly correlated region. Our models also generalize to unseen types of molecules and overcome self-interaction error.

==> custom_macro.tex <==
\usepackage{xcolor}
\newcommand{\todo}[2]{\textcolor{red}{TODO(#1): #2}}
\newcommand{\note}[2]{\textcolor{blue}{NOTE(#1): #2}}

\DeclareMathOperator*{\argmin}{arg\,min}

\def\n{n}
% Standard subscripts
\def\sss{\scriptscriptstyle\rm}
\def\ks{_{\sss KS}}
\def\dmrg{_{\sss DMRG}}
\def\lda{^{\sss LDA}}
\def\gga{^{\sss GGA}}
\def\target{_{\rm target}}
\def\x{_{\sss X}}
\def\c{_{\sss C}}
\def\s{_{\sss S}}
\def\xc{_{\sss XC}}
\def\xctheta{_{\sss XC,\theta}}
\def\xck{_{\sss XC,k}}
\def\xci{_{\sss XC,i}}
\def\Hx{_{\sss HX}}
\def\Hxc{_{\sss HXC}}
\def\H{_{\sss H}}
\def\ee{_{\rm ee}}
\def\br{{\bf r}}
